Extending Segment Anything Model into Auditory and Temporal Dimensions for Audio-Visual Segmentation

Audio-visual segmentation (AVS) aims to segment sound sources in the video sequence, requiring a pixel-level understanding of audio-visual correspondence. As the Segment Anything Model (SAM) has strongly impacted extensive fields of dense prediction problems, prior works have investigated the introduction of SAM into AVS with audio as a new modality of the prompt. Nevertheless, constrained by SAM's single-frame segmentation scheme, the temporal context across multiple frames of audio-visual data remains insufficiently utilized. To this end, we study the extension of SAM's capabilities to the sequence of audio-visual scenes by analyzing contextual cross-modal relationships across the frames. To achieve this, we propose a Spatio-Temporal, Bidirectional Audio-Visual Attention (ST-BAVA) module integrated into the middle of SAM's image encoder and mask decoder. It adaptively updates the audio-visual features to convey the spatio-temporal correspondence between the video frames and audio streams. Extensive experiments demonstrate that our proposed model outperforms the state-of-the-art methods on AVS benchmarks, especially with an 8.3% mIoU gain on a challenging multi-sources subset.

==> tables/table_2_SAM_wo_audio.tex <==
\begin{table}[t]
  \resizebox{\linewidth}{!}{%
    \centering
    \small
    \begin{tabular}{l|cccc}
    \hline
     \multirow{2}{*}{Methods} & \multicolumn{2}{c}{S4} & \multicolumn{2}{c}{MS3}  \\ \cline{2-5} 
      & mIoU      & F-score    & mIoU      & F-score \\ \hline
    SAM with GT (1 Point) & 42.45 & 0.637 & 33.01 & 0.523   \\
    SAM with GT (3 Points) & 68.57 & 0.839 & 54.51 & 0.701   \\
    SAM with GT (Box) & 76.01 & 0.867 & 63.46 & 0.713   \\
    SAM with GT (Boxes) & 76.75 & 0.874 & 66.76 & \textbf{0.813}    \\
    \rowcolor[HTML]{EFEFEF}
    SAM + ST-BAVA (Ours) & \textbf{82.46} & \textbf{0.906} & \textbf{69.01} & 0.775 \\ \hline
    \end{tabular}
  }
  \caption{Quantitative comparison with zero-shot performance of SAM. As vanilla SAM does not support the audio prompt, it receives point or box prompts guiding the region of the sound sources extracted from the ground-truth mask.}
  \label{tab:vanilla_SAM}
  \vspace{-3mm}
\end{table}

==> tables/table_3_abl_feature_fusion.tex <==
\begin{table}[t]
  \resizebox{\linewidth}{!}{%
    \centering
    \small
    \begin{tabular}{l|cccc}
    \hline
     \multirow{2}{*}{Methods} & \multicolumn{2}{c}{S4} & \multicolumn{2}{c}{MS3}  \\ \cline{2-5} 
      & mIoU      & F-score    & mIoU      & F-score \\ \hline
    SAM w/o fusion module  & 81.53 & 0.886 & 63.14 & 0.691   \\
    SAM + CMRAN~\cite{xu2020cross} & - & - & -  & -    \\
    SAM + HAN~\cite{tian2020unified} & -  & -  & -  & -    \\
    SAM + TPAVI~\cite{zhou2022audio} & 81.68 & 0.902 & 64.78 & 0.749   \\
    \rowcolor[HTML]{EFEFEF}
    SAM + ST-BAVA (Ours) & \textbf{82.46} & \textbf{0.906} & \textbf{69.01} & \textbf{0.775} \\ \hline
    \end{tabular}
  }
  \caption{Comparison with different intermediate feature fusion modules inserted into SAM. 
  % Adapter~\cite{liu2023annotation} is not used here for fair comparison.
  }
  \label{tab:abl_feature_fusion}
  \vspace{-3mm}
\end{table}
